Simplified and Space-Optimal Semi-Streaming for $(2+\epsilon)$-Approximate Matching

In a recent breakthrough, Paz and Schwartzman (SODA'17) presented a single-pass ($2+\epsilon$)-approximation algorithm for the maximum weight matching problem in the semi-streaming model. Their algorithm uses $O(n\log^2 n)$ bits of space, for any constant $\epsilon>0$. We present two simplified and more intuitive analyses, for essentially the same algorithm, which also improve the space complexity to the optimal bound of $O(n\log n)$ bits --- this is optimal as the output matching requires $\Omega(n\log n)$ bits. Our analyses rely on a simple use of the primal-dual method and a simple accounting method.

==> improved-mwm.tex <==
\section{Simpler, Improved Analysis via LP Duality}
%We consider the following algorithm of Ghaffari \cite{ghaffari2017space}, improving the space requirements of the algorithm of Paz and Schwartzman \cite{paz20172+}.

%\begin{algorithm}
%	\caption{The Optimal-Space Algorithm}
%	\label{alg:space-optimal}
%	\begin{algorithmic}[1]
%		\medskip
%		\STATE Set $S\leftarrow $ empty stack.
%		\STATE Set $\vec{\phi}\leftarrow \vec{0}_{|V|}$.		
%		\FORALL{$v\in V$}
%			\STATE set $Q(v)\leftarrow $ empty queue.
%		\ENDFOR
%		\FORALL{edges $e=(u,v)$}
%			\IF{$w_e \leq (1+\eps)\cdot (\phi_u+\phi_v)$} \label{line:covered}
%				\STATE \textbf{continue.}
%			\ENDIF
%			\STATE set $w'_e\leftarrow w_e - (\phi_u+\phi_v)$.
%			\STATE\label{line:phi_u} $\phi_u \leftarrow \phi_u + w'_e$.
%			\STATE\label{line:phi_v} $\phi_v \leftarrow \phi_v + w'_e$.
%			\STATE $S.push(e)$.
%			\FORALL{$v\in e$}
%				\STATE $Q(v).enque(e)$.
%				\IF{$|Q(v)|\geq \beta = \frac{3\log(1/\eps)}{\eps}+1 \geq \frac{2\log(1/\eps)}{\log(1+\eps)}+1$}\label{line:big-queue-start}
%					\STATE $e'\leftarrow Q(v).dequeue()$.
%					\STATE remove $e'$ from the stack $S$.\label{line:big-queue-end}
%				\ENDIF
%			\ENDFOR 
%		\ENDFOR 
%		\STATE{}
%		\STATE $M\leftarrow \emptyset$.
%		\WHILE{$S\neq \emptyset$}
%			\STATE $e\leftarrow S.pop()$.
%			\IF{$M\cap N(e)=\emptyset$}		
%				\STATE $M\leftarrow M\cup \{e\}$.
%			\ENDIF
%		\ENDWHILE
%	\end{algorithmic}
%\end{algorithm}

The space usage of this algorithm is immediate, due to each vertex $v\in V$ having an  $O(\log(1/\eps)/\eps)$-sized queue $Q(v)$ associated with it (and $S$ being the union of these queues).

\begin{lem}
	For any fixed $\eps$, Algorithm \ref{alg:OptSpaceAlg} requires $O(n)$ space.
\end{lem} 

\begin{comment}
We now give a simple proof via LP duality that Algorithm \ref{alg:OptSpaceAlg} outputs a  $2(1+O(\eps))$-approximate MWM. To this end, we first make the following observation, showing that the variables $\phi_v$ at the end of the algorithm's run form an approximate feasible dual solution to the LP relaxation of the MWM problem, given in Figure \ref{fig:mwm-lp}.

\begin{figure}[h]
	\begin{small}
		\begin{center}
			\begin{tabular}{rl|rl}
				\multicolumn{2}{c|}{Primal (Packing)} & \multicolumn{2}{c}{Dual
					(Covering)} \\ \hline  
				maximize & $\sum_{e\in E} w_{e}\cdot x_{e}$ &
				minimize & $\sum_{v\in V}{\phi_v}$ \\
				subject to: & & subject to: & \\
				
				$\forall v\in V$: &  $\sum_{e\ni v}x_{e} \leq 1$ &
				$\forall (u,v)\in E$: & $\phi_u + \phi_v \geq w_{(u,v)}$ \\
				
				$\forall e\in E$: & $x_{e} \geq 0$ & $\forall v\in V$: & $\phi_v \geq0$
			\end{tabular}
		\end{center}
	\end{small}
	\vspace{-0.4cm}	
	\caption{The LP relaxation of MWM and its dual}
	\label{fig:mwm-lp}
\end{figure} 
\vspace{-0.4cm}	

\begin{obs}\label{obs:approx-dual}
	The variables $\{\phi_v\}_{v\in V}$ scaled up by $1+\eps$ form a feasible dual solution.
\end{obs}
\begin{proof}
	Each edge $e=(u,v)\in E$ either has it its dual constraint satisfied by $(1+\eps)\cdot \vec{\phi}$ after inspection; i.e., $w_e\leq (1+\eps)\cdot (\phi_u + \phi_v)$. This constraint is  either satisfied before $e$ is inspected or after lines \ref{line:phi_u} and \ref{line:phi_v}, following which $w_e \leq \phi_u + \phi_v \leq (1+\eps)\cdot (\phi_u + \phi_v)$. As the $\phi_v$'s are monotonically increasing, each dual constraint is satisfied by $(1+\eps)\cdot \vec{\phi}$.
\end{proof}
By LP duality, the above implies the following upper bound on the optimal matching.
\begin{cor}\label{cor:phi_ub_MWM}
	The weight of the MWM $M^*$ satisfies $w(M^*) \leq OPT(LP) \leq (1+\eps)\cdot \sum_v \phi_v$.
\end{cor}

We now show that the matching $M$ output by the algorithm has weight at least $w(M)\geq \frac{1}{2(1+O(\eps))}\cdot \sum_{v\in V} \phi_v$, which together with Corollary \ref{cor:phi_ub_MWM}, will imply its approximation ratio. 
%\end{comment}

Denote by $\Delta\phi^e$ the change to $\sum_{v\in V} \phi_v$ in Lines \ref{line:phi_u} and \ref{line:phi_v} of the algorithm during the inspection of edge $e$. (Note that $\Delta \phi^e=0$ if the algorithm does not reach these lines when inspecting edge $e$ due to the test in Line \ref{line:covered}.) By definition, by the algorithm's termination, $\sum_v \phi_v = \sum_e \Delta \phi^e$. The following lemma relates the weight of an edge $e$ to $\Delta\phi^{e'}$ of previously-inspected edges $e'$ neighboring $e$.

\begin{lem}\label{lem:weight-vs-dual-change}
	For all edge $e\in E$ added to the stack $S$, if we denote its preceding neighboring edges by $\mathcal{P}(e)=\{e'\in N^+(e) \mid e' \mbox{ inspected no later than } e\}$, then $$w_e \geq \frac{1}{2}\cdot \sum_{e'\in \mathcal{P}(e)} \Delta\phi^{e'} = \sum_{e'\in \mathcal{P}(e)} w'_{e'}.$$
\end{lem}
\begin{proof}
	First, we note that $\Delta\phi^e = 2w'_e$, due to Lines \ref{line:phi_u} and \ref{line:phi_v}, or put otherwise $w'_e=\frac{1}{2}\cdot \Delta\phi^e$. On the other hand, if we denote by $\phi_u^e$ and $\phi_v^e$ the values of $\phi_u$ and $\phi_v$ before 
	the inspection of $e$, respectively, we have that $\phi_u^e + \phi_v^e \geq \frac{1}{2}\cdot  \sum_{e'\in \mathcal{P}(e)\setminus \{e\}} \Delta\phi^{e'}$, where this inequality is an equality unless $G$ contains edges parallel to $e$. Consequently, we have that indeed 
	\begin{align*}
		w_e & = w'_e + (\phi_u^e + \phi_v^e) \geq \frac{1}{2}\cdot \sum_{e'\in \mathcal{P}(e)} \Delta \phi^{e'} = \sum_{e'\in \mathcal{P}(e)} w'_{e'}. \qedhere
	\end{align*}
\end{proof}

Lemma \ref{lem:weight-vs-dual-change} combined with Corollary \ref{cor:phi_ub_MWM} are sufficient to prove that the above algorithm without the limiting of queue sizes in Lines \ref{line:big-queue-start}-\ref{line:big-queue-end} outputs a $2(1+\eps)$-approximate MWM, since they imply that $\sum_{e \in M}w_e \geq \frac{1}{2}\sum_e \Delta\phi^e = \frac{1}{2}\sum_v \phi_v \geq \frac{1}{2(1+\eps)}\cdot w(M^*)$. 
%\end{comment}

We now address the loss due to Lines \ref{line:big-queue-start}-\ref{line:big-queue-end}, starting with the following recursive definition.

\begin{Def}
	We say an edge $e'$ which was inserted into $S$ was \emph{discarded} if it was later removed from $S$,
	and say the edge was \emph{kept} otherwise.
	We say a discarded edge $e'$ was \emph{discarded by} a kept edge $e$ if $e'$ is removed from $S$ in Lines \ref{line:big-queue-start}-\ref{line:big-queue-end} during the inspection of edge $e$, or during the inspection of an edge $e''$ which is in turn discarded by $e$. We denote the set of edges discarded by $e$ by $\mathcal{D}(e)$.
\end{Def}

\begin{lem}\label{lem:weight-discarded}
	For all $\eps\leq 1/4$, for each edge $e\in E$, we have $w'_e\geq \frac{1}{4\eps}\cdot \sum_{e'\in \mathcal{D}(e)} w'_{e'}$.
\end{lem}
%In order to prove this lemma, we rely on the following simple observation, that the weights of edges enqued into $Q(v)$ increase exponentially.
%\begin{obs}	
%	
%\end{obs}

\begin{proof} %[Proof of Lemma \ref{lem:weight-discarded}]
	The number of edges of $\mathcal{D}(e)$ discarded upon inspection of $e$ is at most two -- one for each endpoint of $e$. Let $\phi_v^e$ be the value of $\phi_v$ prior to the inspection of $e$. Then, we have $w'_e\geq \eps\cdot (\phi_u^e+\phi_v^e) \geq \eps\cdot  \phi_v^e$. Moreover, as $\phi_v$ increases by at least a factor of $(1+\eps)$ following each inspection of an edge neighboring $v$, we have that each edge $e'$ discarded when $e$ was inspected has $w'$-value at most $w'_{e'}\leq 1/(1+\eps)^{\beta} \cdot \phi_v^e \leq  \eps^2\cdot (1/\eps)\cdot w'_e = \eps\cdot w'_e$.
	Similarly, each of the above two edges discarded directly by $e$ can be directly responsible for the discarding of four edges in $\mathcal{D}(e)$, of $w'$-value at most $\eps\cdot w'_{e'}\leq \eps^2 \cdot w'_{e}$ each. Generally, the edges of $\mathcal{D}(e)$ can be partitioned into sets of at most $2^i$ edges each, of $w'$-value at most $\eps^{i}\cdot w'_e$, for all $i\in \mathbb{N}$. Summing over all these sets, we find that indeed
	\begin{align*}
		\sum_{e'\in \mathcal{D}(e)} w'_{e'} & \leq \sum_{i=1}^\infty (2\eps)^i\cdot w_e \leq 4\eps \cdot w'_e. \qedhere
	\end{align*}
\end{proof}
%\end{comment}
Armed with Lemmas \ref{lem:weight-vs-dual-change} and \ref{lem:weight-discarded}, we now prove our main theorem.

\begin{thm}
	For all $\eps\leq \frac{1}{4}$, 
	Algorithm \ref{alg:OptSpaceAlg} is $2(1+6\eps)$-approximate.
\end{thm}
\begin{proof}
	By Lemma \ref{lem:weight-vs-dual-change}, for each edge $e\in M$, we have
%	\begin{equation}\label{eqn:w_e-lb}
		$w_e \geq  \sum_{e'\in \mathcal{P}(e)} w'_{e'}.$
%	\end{equation}	
	On the other hand,  by Lemma \ref{lem:weight-discarded}, we have that 
%	\begin{equation}\label{eqn:w_e-lb-discarded}
		 $4{\eps}\cdot w'_e \geq  \sum_{e'\in \mathcal{D}(e)} w'_{e'}.$
%	\end{equation}
%	 Combining these inequalities, Inequalities \ref{eqn:w_e-lb} and \ref{eqn:w_e-lb-discarded},
 we find that 		 
	\begin{align*}
		w_e \cdot (1+4\eps) &  \geq \sum_{e'\in \mathcal{P}(e)} \big( w'_{e'} +  \sum_{e''\in \mathcal{D}(e')} w'_{e''} \big).
	\end{align*}
	
	But each kept edge $e'$ not added to $M$ is due to a kept edge $e$ added to $M$; that is, some $e$ such that $e'\in \mathcal{P}(e)$. Likewise, each discarded edge is discarded due to some kept edge. Consequently, the right hand side of the above expression summed over all edges of the output matching $M$ is precisely $\sum_{e'\in E} w'_{e'} = \frac{1}{2}\cdot \sum_{e'\in E} \Delta\phi^{e'} = \frac{1}{2}\cdot \sum_{v\in V} \phi_v$, which by Corollary \ref{cor:phi_ub_MWM}, yields
	\begin{align*}
		\sum_{e\in M} w_e & \geq \frac{1}{2(1+4\eps)} \cdot \sum_{v\in V} \phi_v \geq \frac{1}{2(1+4\eps)(1+\eps)}\cdot w(M^*) \geq \frac{1}{2(1+6\eps)}\cdot w(M^*).\qedhere 
	\end{align*}
\end{proof}
\end{comment}


==> intro.tex <==
\section{Introduction and Related Work}
The maximum weight matching (MWM) problem is a classical optimization problem, with diverse applications, which has been studied extensively since the 1965 work of Edmonds \cite{edmonds1965paths}. Naturally, this problem has received significant attention also in the \emph{semi-streaming} model. This is a modern model of computation, introduced by Feigenbaum et al.\cite{feigenbaum2005graph}, which is motivated by the need for processing massive graphs whose edge set cannot be stored in memory. In this model, roughly speaking, the edges of the graph arrive in a stream, and the algorithm should process this stream and eventually output its solution --- a matching in our case --- while using a small memory at all times. Ideally, this memory size should be close to what is needed for keeping just the output. More formally, the setting of the MWM problem in the semi-streaming matching is as follows.

\paragraph{MWM in the Semi-Streaming Model} Let $G=(V, E, w)$ be a simple graph with non-negative edges weights $w:E\rightarrow \mathbb{R}_{>0}$. Let $n=|V|$, $m=|E|$. We assume that the edge weights are normalized so that the minimum edge weight is $1$ and we use $W$ to denote the maximum edge weight. In the semi-streaming model, the input graph $G$ is provided as a stream of edges. In each iteration, the algorithm receives an edge from the stream and processes it. The algorithm has a memory much smaller than $m$ and thus it cannot store the whole graph. The amount of the memory that the algorithm uses is called its \emph{space complexity} and we wish to have it as small as possible. The objective in the semi-streaming \emph{maximum weight matching} (MWM) problem is that, at the end of the stream, the algorithm outputs a matching, whose weight is close to the weight of the maximum weight matching. 



\paragraph{State of the Art} There has been a sequence of successively improved approximation algorithms for MWM in the semi-streaming model. Feigenbaum et al.~gave a $6$ approximation\cite{feigenbaum2005graph}, McGregor gave a $5.828$ approximation\footnote{He also presented a $2+\eps$ approximation, but using $O(1/\eps^3)$ passes on the input.}\cite{mcgregor2005finding}, Epstein et al. gave a $4.911+\eps$ approximation\cite{epstein2011improved}, Crouch and Stubbs gave a $4+\eps$ approximation\cite{crouch2014improved}, and Grigorescu et al.~improved this bound to $3.5+\eps$\cite{grigorescu2016streaming}. However, these approximations remained far away from the more natural and more familiar $2$ approximation, which the sequential greedy method provides. 

In a recent breakthrough, Paz and Schwartzman\cite{PS17-StreamingMatching} presented a truly simple algorithm that achieves an approximation of $2+\eps$ for any constant $\eps>0$, using $O(n\log^2 n)$ bits of space. More concretely, the algorithm maintains $O(n\log n)$ edges, while working through the stream, and at the end, it computes the matching using these maintained edges.


\paragraph{Our contribution} We present alternative analyses for (a slight variant of) the algorithm of Paz and Schwartzman, which have two advantages: (1) they imply that keeping merely $O(n)$ edges suffices, and thus improve the space complexity to $O(n\log n)$ bits, which is optimal, (2) they provide a more intuitive and also more flexible accounting of the approximation. 

Concretely, Paz and Schwartzman\cite{PS17-StreamingMatching} used an extension of \emph{the Local Ratio theorem}\cite{bar2001unified, bar2004local} to analyze their algorithm. We instead present two different, simpler, arguments, which are more flexible and allow us to improve the space-complexity to obtain the optimal space bound. Our analyses rely on the primal dual method and an intuitive \emph{blaming} argument.

\paragraph{Roadmap} In \Cref{sec:review}, as a warm up, we review (a simple version of) the algorithm of Paz and Schwartzman. In \Cref{sec:Analysis}, we present an simpler and more intuitive style of analysis for this algorithm. In \Cref{sec:improve}, we present the improved algorithm that achieves a space complexity of $O(n\log n)$, the analysis of which relies crucially on the flexibility of the analyses presented in \Cref{sec:Analysis}. Throughout, we present both alternative proofs, explicitly noting whether the proof is duality-based or blaming-based. \todo{Non-standard. What do you think?}
